Minimax Regret Optimisation for Robust Planning in Uncertain Markov Decision Processes

The parameters for a Markov Decision Process (MDP) often cannot be specified exactly. Uncertain MDPs (UMDPs) capture this model ambiguity by defining sets which the parameters belong to. Minimax regret has been proposed as an objective for planning in UMDPs to find robust policies which are not overly conservative. In this work, we focus on planning for Stochastic Shortest Path (SSP) UMDPs with uncertain cost and transition functions. We introduce a Bellman equation to compute the regret for a policy. We propose a dynamic programming algorithm that utilises the regret Bellman equation, and show that it optimises minimax regret exactly for UMDPs with independent uncertainties. For coupled uncertainties, we extend our approach to use options to enable a trade off between computation and solution quality. We evaluate our approach on both synthetic and real-world domains, showing that it significantly outperforms existing baselines.

==> tex/broader_impact.tex <==
%!TEX root = ./neurips_2020.tex

\section*{Broader Impact}
Automated decision making using MDPs estimated from data may perform much worse than expected due to model uncertainty~\cite{mannor2004bias}.
%
In some application domains, for example robot navigation with limited battery life~\cite{lacerda2019probabilistic}, unanticipated poor performance may result in undesirable outcomes.
%
As such, automated decision making systems should take into account model uncertainty.

From a decision science perspective, uncertainty can be categorised as \textit{ambiguity} or \textit{risk}~\cite{ellsberg1961risk}.
%
Ambiguity (also called Knightian uncertainty) is uncertainty for which the likelihood of different outcomes cannot be quantified, whereas risk is quantifiable uncertainty.
%
Optimising for the worst-case expected value or regret over all plausible models is ambiguity-averse.
%
However, both the minimax expected value and minimax regret criteria are based on expected values and are therefore risk-neutral.
%
This is a natural objective for  applications in which the MDP is executed many times, where the fluctuation in cost averages out over many executions.
%
In situations where mitigating risk due to fluctuation over individual runs is important, Risk-Sensitive MDPs~\cite{howard1972risk} and Constrained MDPs~\cite{altman1999constrained} are suitable alternatives. 

Most research on planning for UMDPs has addressed optimising for the worst-case expected value with independent uncertainties~\cite{iyengar2005robust, nilim2005robust, wiesemann2013robust}. However, the resulting policies may be very conservative and perform poorly for the majority of possible scenarios~\cite{delage2010percentile}. Therefore, optimising for the worst-case expected value may be undesirable for many applications. In this work, we have addressed minimax regret planning which is a promising alternative as it is:  intuitive to understand, robust to model uncertainty by minimising the worst-case sub-optimality, and is less conservative than optimising for the worst-case expected value.


==> tex/corrigendum_v1.tex <==
\section{Corrigendum}
In the subsection ``Exact Solution for Independent Uncertainties'', we originally claimed that if the uncertainty set was independent, then Problem 2 can be solved exactly by applying Algorithm 1 with $n = 1$. However, we now realise that even for independent uncertainty sets, our method is approximate.

As stated in Proposition~\ref{prop:creg}, the regret for a policy can be computed using the Bellman equation
\begin{equation*}
	reg(s, \pi) = \sum_{a \in A} \pi(s, a) \cdot \\ \big[Q^{gap}(s, a) + \sum_{s' \in S}T(s, a, s')\cdot reg(s', \pi) \big], \hspace{5pt} \normalsize{\textit{where}}
\end{equation*}

\begin{equation*}
	Q^{gap}(s, a) = \big[ \bar{C}(s, a) + \sum_{s' \in S}T(s, a, s') \cdot V(s', \pi^*) \big] - V(s, \pi^*).
\end{equation*}

The maximum regret over all uncertainty samples, $\xi_q \in \xi$,  is therefore
\begin{multline*}
	\max_{\xi_q \in \xi} reg_q(s, \pi) = \max_{\xi_q \in \xi} \Bigg\{ \sum_{a \in A} \pi(s, a) \cdot  \Big[Q^{gap}_q(s, a) + \sum_{s' \in S}T_q(s, a, s')\cdot reg_q(s', \pi) \Big] \Bigg\} 
	\\
	= \max_{\xi_q \in \xi} \Bigg\{ \sum_{a \in A} \pi(s, a) \cdot \Big[\bar{C}_q(s, a) + \sum_{s' \in S}T_q(s, a, s') \cdot V_q(s', \pi^*_q) - \bar{C}_q(s, \pi_q^*(s)) -
	\\
	\sum_{s' \in S}T_q(s, \pi_q^*(s), s') \cdot V_q(s', \pi^*_q) + \sum_{s' \in S}T_q(s, a, s')\cdot reg_q(s', \pi) \Big] \Bigg \}
\end{multline*}

For independent uncertainty sets we can separately maximise over the uncertainty set to applied at the current step, $\xi_q$, and the uncertainty set to be applied at all subsequent steps, $\xi_{q'}$:

\begin{multline}
	\label{eq:reg_err1}
	\max_{\xi_q \in \xi} reg_q(s, \pi) = \max_{\xi_q, \xi_{q'} \in \xi} \Bigg\{ \sum_{a \in A} \pi(s, a) \cdot \Big[\bar{C}_q(s, a) + \sum_{s' \in S}T_q(s, a, s') \cdot V_{q'}(s', \pi^*_{q'}) - \bar{C}_q(s, \pi_q^*(s)) -
	\\
	\sum_{s' \in S}T_q(s, \pi_q^*(s), s') \cdot V_{q'}(s', \pi^*_{q'}) + \sum_{s' \in S}T_q(s, a, s')\cdot reg_{q'}(s', \pi) \Big] \Bigg \}
\end{multline}


However, when performing minimax value iteration using Algorithm 1 with $n = 1$, the $V_{q'}$ terms in Equation~\ref{eq:reg_err1} are approximated with $V_q$. This enables a separate maximisation over $\xi_{q'}$ to maximise the regret at the successor states:
\begin{multline}
	\max_{\xi_q \in \xi} reg_q(s, \pi)  \approx \max_{\xi_q \in \xi} \Bigg\{ \sum_{a \in A} \pi(s, a) \cdot \Big[\bar{C}_q(s, a) + \sum_{s' \in S}T_q(s, a, s') \cdot V_{q}(s', \pi^*_q) - \bar{C}_q(s, \pi_q^*(s)) -
	\\
	\sum_{s' \in S}T_q(s, \pi_q^*(s), s') \cdot V_{q}(s', \pi^*_q) + \max_{\xi_{q'} \in \xi} \sum_{s' \in S}T_q(s, a, s')\cdot reg_{q'}(s', \pi) \Big] \Bigg \}
\end{multline}

Because of this approximation of the $V_{q'}$ terms with $V_q$ in our dynamic programming approach, our approach only approximately optimises the maximum regret for problems with independent uncertainty sets.
